BoPF: Mitigating the Burstiness-Fairness Tradeoff in Multi-Resource Clusters

Simultaneously supporting latency- and throughout-sensitive workloads in a shared environment is an increasingly more common challenge in big data clusters. Despite many advances, existing cluster schedulers force the same performance goal - fairness in most cases - on all jobs. Latency-sensitive jobs suffer, while throughput-sensitive ones thrive. Using prioritization does the opposite: it opens up a path for latency-sensitive jobs to dominate. In this paper, we tackle the challenges in supporting both short-term performance and long-term fairness simultaneously with high resource utilization by proposing Bounded Priority Fairness (BoPF). BoPF provides short-term resource guarantees to latency-sensitive jobs and maintains long-term fairness for throughput-sensitive jobs. BoPF is the first scheduler that can provide long-term fairness, burst guarantee, and Pareto efficiency in a strategyproof manner for multi-resource scheduling. Deployments and large-scale simulations show that BoPF closely approximates the performance of Strict Priority as well as the fairness characteristics of DRF. In deployments, BoPF speeds up latency-sensitive jobs by 5.38 times compared to DRF, while still maintaining long-term fairness. In the meantime, BoPF improves the average completion times of throughput-sensitive jobs by up to 3.05 times compared to Strict Priority.

==> scripts/background.tex <==
\section{Existing scheduling policies on Yarn}

\desc{Fair Scheduler and Capacity Scheduler in Yarn}

Essentially, Yarn allocates the resources to its active queues. An queue is called active, if there is at least one job. In Yarn, there are two types of schedulers, which are Capacity Scheduler (CS) and Fair Scheduler (FS). Fair Scheduler equally splits cluster resources among the active queues [?]. Meaning, Fair Scheduler pursue the fairness among the queues. In the meantime, Capacity Scheduler is designed to guarantee the resource capacity for each tenant [?]. In addition, There is an added benefit that an organization can access the available resources, which are not used by others. As we bridge the gap that the interactive users are not satisfied with both existing schedulers, we discuss why Fair Scheduler and Capacity Scheduler do not work well on this gap.

\desc{How Fair Scheduler works? Why do we need a new scheduling policy?}

Fair Scheduler organizes the arrival jobs into queue (more precisely, pools), and fairly divides resources between the queues. The queues can be hierarchal in which the same level queues are to receive the same amount of resources. In addition, jobs can be scheduled within a queue. There are 3 fair scheduling policies in Fair Scheduler: First in first out (FIFO), fair, and dominant resource fairness (DRF). 

\begin{itemize}
\item FIFO: FIFO scheduling policy allocates the resource to the coming jobs based on their priorities and arrival times.
\end{itemize}


Fair Scheduler + weight.

Capacity Scheduler.



==> scripts/implememtation.tex <==
\section{Implementation}

We implement our solution on Yarn Scheduler of Hadoop 2.7.2 \cite{yarn}. The solution design is broken down into two steps, which are \emph{admission control} for the applications and \emph{resource allocation for the excess resource} among the queues. We suppose that each queue represents for a tenant or a type of applications, which have different minimum requirement on resource.

Is minimum resource requirement is necessary for cloud provider? Some applications like Flink requires resource to be ready before running. Iteratively, it keeps asking for more containers until it is satisfied. If it is not satisfied, it does not only waste the resource for nothing but also block the other queued applications. Instead, we offer tenant to indicate their minimum resource requirement. If the application is not satisfied, it is held in the queue and makes resource free for other applications. 

What does minimum resource requirement benefit tenants? By indicating the minimum resource requirement, tenants have more control on their application performance. For instance, tenants can estimate the worst-case performance for their cloud computing jobs based on the minimum resource requirement.

\subsection*{Admission control}

\emph{Minimum resource requirement} is configured for each queue, which represents for each tenant's requirement. To implement this parameter on the Hadoop 2.7.2, we add a property \textit{minReq} to \textit{Queue} class. The default value of \textit{minReq} is zero for the tenants are flexible on resource demand. By this way, all the applications in the same queue require the same minimum amount of resource to complete their tasks. Once the minimum resource is satisfied, the application can be scheduled. Otherwise, it is queued until the cluster has enough resource.

Admission control is to admit as many applications as possible. On the other hand, application's minimum resource requirement must be satisfied. After an application is SUBMITTED to a queue, the scheduler creates an application attempt (AppAttempt) to request the necessary resource. If resource is available for the AppAttempt, it is SCHEDULED to obtain the resource containers. If the cluster resource is not available, the AppAttempt state is set at WAITED to try again.

One important modification on Yarn is to determine whether resource is available for an AppAttempt before scheduling. To do this, we need to compute the resource usage for admission. In the a cluster, the resources are distributed the nodes, it is difficult to determined the amount of resource are used in real time. Although we can do it, it may result in  a deadlock when there are more than one AppAttempt acquiring the resources. Instead, we can determine how much resource are reserved by the running queues. A running queue is a queue that has at least one AppAttempt SCHEDULED to run. 

Is there possible deadlock when scheduling the applications? Yes, it can happen if more than two queues need the resource and update their states a the same time. To prevent the deadlock, we make sure that the states of queues cannot be updated in the same time. People may argue that this could lead to performance degradation. However, the updating processes happens in the master node which last shortly.

\subsection*{Resource allocation for excess resource}

The second step is how to allocate the remaining resource after admission control. A simple solution is to share the resource among the queues by using DRF.

==> scripts/multiple_LQ_sim.tex <==
\subsubsection{Admission control for Multiple LQs}
\label{sec:admission_sim}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/res_usage_b1i3_legend} 
    \vspace{-0.2cm}
    \subfloat[DRF: \burstq-0, \burstq-1, \burstq-2 are unhappy with high latency.]{\includegraphics[width=0.8\linewidth]{fig/b1i3_res_usage_drf} \label{fig:admission_drf}} 
    \vspace{-0.1cm}
    \subfloat[SP: \batchq-0 is starving of resources.]{\includegraphics[width=0.8\linewidth]{fig/b1i3_res_usage_strict} \label{fig:admission_strict}}
    \vspace{-0.1cm}            
    \subfloat[N-\name: Only {\burstq}-0 and {\batchq}-0 are happy.]{\includegraphics[width=0.8\linewidth]{fig/b1i3_res_usage_Hard} \label{fig:admission_hard}}
    \vspace{-0.1cm}    
    \subfloat[\name: {\burstq}-0, {\burstq}-1 and {\batchq}-1 are happy.]{\includegraphics[width=0.8\linewidth]{fig/b1i3_res_usage_speedfair} \label{fig:admission_speedfair}}
    \vspace{-0.1cm}    
    \caption{[Simulation] DRF and SP fail to guarantee both performance and fairness simultaneously. \name gives the best performance to \burstq-0, near optimal performance for \burstq-1, and maintains fairness among 4 queues. \burstq-2 requires too much resource, so its performance cannot be guaranteed.}
    \vspace{-0.5cm}    
    \label{fig:admission_control}
\end{figure}


To demonstrate how \name works with multiple {\burstq}s, we set up 3 {\burstq}s (\burstq-0, \burstq-1, and \burstq-2) and a single \batchq (TQ-0).
The jobs \batchq-0 are queued up at the beginning while \burstq-0, \burstq-1, and \burstq-2 arrive at 50, 100, and 150 seconds, respectively.
The periods of {\burstq}-0, {\burstq}-1, and {\burstq}-2 are 150, \diff{110}, and 60 secs. All the {\burstq}s jobs have the identical demand and task durations.
The TQ jobs are chosen from the BB benchmark.
\name admits {\burstq}-0 to the Hard Guarantee class, {\burstq}-1 to the Soft Guarantee class, and {\burstq}-2 to the Elastic class.

Figure \ref{fig:admission_control} shows the resource usage (CPU and memory) for each queue across four schedulers, i.e., DRF, SP, N-\name and \name.
The capacity of CPU or memory is 1000 nodes.
As an instantaneously fair scheduler, DRF continuously maintains the fair share for all queues as in Figure \ref{fig:admission_drf}.
Since \burstq-2 requires a lot of resources, SP makes \batchq-0 starving for resources (Figure \ref{fig:admission_strict}). N-\name provides \burstq-0 with resource guarantee and it fairly share the resources to \burstq-1, \burstq-2, and \batchq-0 (Figure \ref{fig:admission_hard}).
\name provides hard guarantee to \burstq-0 and soft guarantee to \burstq-1 as in Figure \ref{fig:admission_speedfair}.
The soft guarantee allows \burstq-1 performs better than using N-\name.
Since \burstq-2 demands too much resources, \name treats it like \batchq-0.

Figure \ref{fig:avg_multi_queue} shows the average completion time of jobs on each queue across the four schedulers.
The performance of DRF for \burstq jobs is the worst among the four schedulers but it is the best for only \batchq-0.
The performance of SP is good for \burstq jobs but it is the worst for \batchq jobs.
N-\name provides the best performance for \burstq-0 but not \burstq-1 and \burstq-2.
\name is the best among the four schedulers.
The three of four queues, i.e., \burstq-0, \burstq-1, and \batchq-0, significantly benefit from \name.
\name even outperforms SP for \burstq-0 and \burstq-1 jobs and does not hurt any {\batchq}.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/avg_multi_queuesadmit}
    \caption{[Simulation] \name provides with better performance for {\burstq}s than DRF and N-\name. Unlike SP, \name protects the performance of \batchq jobs.}
    \label{fig:avg_multi_queue}
\end{figure}


==> scripts/problem_formulation.tex <==
\section{Problem formulation (by Tan)}

A arbitrary job requires one or many containers, each container is specified a set of resources (CPU, RAM). Here, we can allocate the number of containers to the job. We consider 3 application types: Streaming, Interactive, and Batch as in Table \ref{tbl:application_type}

\begin{table}[!htp]
	\centering
	\begin{tabular}{@{}lll@{}}
		\toprule\addlinespace
		%\multicolumn{3}{l}{Application type} \\
		\textbf{Application type} & & Input \\ \addlinespace
		\cmidrule{1-3}\addlinespace
		\textbf{Streaming}      &  & $\rho$, execution interval (second)\\
		($N_s$ periodic jobs)	&  & $\delta_s$ maximum delay for the first job\\
				&                       & $\alpha_s$ resources per container \\ \addlinespace 

		\textbf{Interactive}    &          & $\tau$, maximum completion time\\
		(1 single job) 			&  						& $\alpha_i$, resource per container \\ \addlinespace
		
		\textbf{Batch}  &          & $T$, max expected completion time\\
		(1 single job)	& 		   &  $\alpha_b$, resource per container\\ \addlinespace
		\bottomrule
	\end{tabular}
	\label{tbl:application_type}
\end{table}

A streaming application is guaranteed to have a small delay ($<\delta_s$) for the first job, while the processing time for the other jobs must be less than the execution time $\rho$. In the meantime, an interactive application prefer to complete the job as soon as possible ($<\tau$). The batch application having a long processing time must predict the expected completion time $T$. 

\subsection{Running example}

We run 3 applications: streaming at $t=0$, interactive at $t=0$, batch at $t=0$. Assume that their containers require the same amount of resources. The cluster capacity is $30$ containers. If each application is allocated with 100\% resource,
$  $\begin{itemize}
	\item A streaming job (among $N$ periodic jobs of the streaming applications) takes 1 sec --> resource needed per job: 30*1 container-secs.
	\item A interactive job takes 1 sec. --> resource needed per job: 30*1 container-secs.
	\item A batch job takes 5 secs. --> resource needed per job: 30*5=150 container-secs.
\end{itemize}
Figure 5, 6 \& 7 illustrate the service curve for each application.

\begin{figure}
\centering
\begin{tikzpicture}[scale=1]
\begin{axis}[
axis lines = left,
xlabel = secs,
ylabel = containters-secs,
xmin=0,xmax=24,
ymin=0,ymax=150,
]
%Below the red parabola is defined
\addplot [
domain=0:3, 
samples=100, 
color=red,
]
{10*x};
\addplot [
domain=3:24, 
samples=100, 
color=red,
]
{30/12*(x-3)+10*3};
\end{axis}
\end{tikzpicture}
\caption{Service curve for the streaming application with $\rho=12,\delta_s=3$. 30 container-secs are allocated in 3 secs for the first job of $N$ streaming jobs meaning the delay for the streaming application is less than 3 secs. In addition, it ensures that the rest $N-1$ jobs can finish in $\rho=12$ secs.}
\end{figure}

\begin{figure}
	\centering
	\begin{tikzpicture}[scale=1]
	\begin{axis}[
	axis lines = left,
	xlabel = secs,
	ylabel = containters-secs,
	xmin=0,xmax=24,
	ymin=0,ymax=150,
	]
	%Below the red parabola is defined
	\addplot [
	domain=0:5, 
	samples=100, 
	color=red,
	]
	{6*x};
	\addplot [
	domain=5:24, 
	samples=100, 
	color=red,
	]
	{6*5};
	\end{axis}
	\end{tikzpicture}
	\caption{Service curve for the interactive application with $\tau=5$. The interactive application is guaranteed to be allocated enough resource to finish in 5 secs. Beyond 5 secs, there is no guarantee that flattens the service curve.}
\end{figure}

\begin{figure}
	\centering
	\begin{tikzpicture}[scale=1]
	\begin{axis}[
	axis lines = left,
	xlabel = secs,
	ylabel = containters-secs,
	xmin=0,xmax=24,
	ymin=0,ymax=150,
	]
	%Below the red parabola is defined
	\addplot [
	domain=0:5, 
	samples=100, 
	color=red,
	]
	{150/150*x};
	\addplot [
	domain=5:24, 
	samples=100, 
	color=red,
	]
	{150/20*(x-5)+150/150*5};
	\end{axis}
	\end{tikzpicture}
	\caption{Service curve for the batch application with $T=24$. This service curve allows the batch job to finish in 24 secs as expected.}
\end{figure}



==> scripts/sensitivity.tex <==
\vsp\subsection{Sensitivity Analysis}
\label{sec:sensitivity_analysis}\vsp

\subsubsection{Impact of estimation errors}
\label{sec:estimation_error_sim}

\name requires users to report their estimated demand for \burstq jobs.
However, it is challenging to estimate the demand accurately, which naturally results in estimation errors.
To understand the impact of estimation errors on \name, we assume that estimation errors $e(\%)$ follow the standard normal distribution with zero mean.
The standard deviation (std.) of estimation errors lines in $[0, 50]$.
To adopt the estimation errors, we update the task demand and durations of \burstq jobs as $ {task}_{new} = {task}_{original}*(1+e/100)$.

Figure \ref{fig:sen_analysis_est_err} shows the impact of estimation errors on the average completion time of \burstq jobs.
There are 1 single \burstq and 8 {\batchq}s.
\burstq jobs arrive every 350 seconds.
\name is robust when the standard deviation of estimation errors vary 0 to 20.
The \burstq jobs in BB suffer more from the large estimation errors (std. $>30$) than that of TPC-DS and TPC-H.
The delays are caused by the underestimated jobs because the excessive demand is not guaranteed by the system.
Meanwhile, the overestimated jobs do not suffer any delays as the guaranteed resource is more than needed.
Although estimation errors result in performance degradation, the performance of \burstq jobs is still much better than that of DRF (162 seconds).
%In the case of large errors, users are suggested reporting larger demands and longer stage-1 durations to improve the performance.\todo{Sentence doesn't parse.}

\begin{figure}[!h]
\centering
    \includegraphics[width=0.7\linewidth]{fig/sen_analysis_est_err}
\caption{[Simulation] \name's performance degrades with larger estimation errors, yet is still significantly better than DRF (162 secs).}
\label{fig:sen_analysis_est_err}
\end{figure}


\subsubsection{Impact of non-preemption}
\label{sec:non_preemption_sim}

To evaluate the impact of non-preemption, we vary the average task durations of {\batchq} jobs.
The longer task duration is, the longer the task holds its resources.
In this evaluation, we set up 1 \burstq and 8 {\batchq}s on the simulator.
Each \burstq job arrives every 350 secs.
The evaluation is run on three workloads BB, TPC-DS, and TPC-H.

\begin{figure}[!h]
\centering
\includegraphics[width=0.7\linewidth]{fig/sen_analysis_task_duration}
\caption{[Simulation] With longer average task durations, the impact of non-preemption on the performance of \burstq jobs becomes larger. However, the average completion time is still significantly better than that of DRF (162 secs).}
\label{fig:sen_analysis_task_duration}
\end{figure}

Figure \ref{fig:sen_analysis_task_duration} shows the impact of average task durations of \batchq jobs on the average completion time of \burstq jobs.
When we increase the average task durations, the performance of \burstq jobs is degraded.
Due to the variations of task durations, the BB curve stops increasing from 20, while the TPC-DS and TPC-H curves keep going up.
Recall the distributions of the task durations in Figure \ref{fig:worklad_cdf}: 70 percent of tasks in BB are very short.
When the average task durations are more than 20 seconds, there are still a large number of short tasks in BB that allows \name to allocate more resources to \burstq jobs.
TPC-DS and TPC-H have more variations of task durations that result in increasing delay for \burstq jobs.
